Approximation Methods for Partially Observed Markov Decision Processes (POMDPs)

POMDPs are useful models for systems where the true underlying state is not known completely to an outside observer; the outside observer incompletely knows the true state of the system, and observes a noisy version of the true system state. When the number of system states is large in a POMDP that often necessitates the use of approximation methods to obtain near optimal solutions for control. This survey is centered around the origins, theory, and approximations of finite-state POMDPs. In order to understand POMDPs, it is required to have an understanding of finite-state Markov Decision Processes (MDPs) in \autoref{mdp} and Hidden Markov Models (HMMs) in \autoref{hmm}. For this background theory, I provide only essential details on MDPs and HMMs and leave longer expositions to textbook treatments before diving into the main topics of POMDPs. Once the required background is covered, the POMDP is introduced in \autoref{pomdp}. The origins of the POMDP are explained in the classical papers section \autoref{classical}. Once the high computational requirements are understood from the exact methodological point of view, the main approximation methods are surveyed in \autoref{approximations}. Then, I end the survey with some new research directions in \autoref{conclusion}.

==> Applications.tex <==
% \chapter{Applications of POMDPs to Varied Research Disciplines}
\section{POMDP Applications}
\label{Applications}
% \section{POMDP Applications Prelude}
In this final section, I briefly review the POMDP model I will be assuming for the rest of this survey paper. This model includes a finite state, action, and observation space. This model is very general and has been applied to solve research problems in a number of fields. Then, I discuss my hierarchy of POMDP research I created after reviewing a few other survey articles and collecting the different application domain examples. The point of this section is to survey the most recent work done in applying POMDPs in various domains. 

% I want to update previous surveys of applications to fill in the last twenty years or so since an article was written on synthesizing the new research areas of POMDPs.

For every area, a few of the problems are put into a tabular form showing one could choose the states, observations and controls. Typically the application area is mentioned, but the states, observations, and controls are not discussed or presented in a compact way.  At the end of this chapter, I will link to some other great earlier survey articles from the 1990s that can provide more context. Nevertheless, my hierarchy and organization of the POMDP applications I am hoping will allow for researchers in several distinct disciplines that have not given POMDPs much thought to start to gain real insight on how to model their problems as POMDPs. If this is achieved, then they can start to extend the POMDP model and develop really useful control policies for their specific problem domain. The main survey article of POMDP Applications I will be extending and basing my extension off of is \cite{cassandra1998survey}.

% After going over my POMDP research hierarchy, I will present each node in the tree by its own table. In each table, I will list for each problem domain what are generally used or intelligent choices for the states, the actions, and the observations, as well as discuss the immediate costs for modeling.

The most active research community for POMDPs is the Artificial Intelligence (AI) community. Some researchers in fields out of the AI community have started to adopt the POMDP paradigm to their problems where hidden state exists, i.e., imperfect state information. The POMDP captures stochastic state transitions, and observation uncertainty. Since the 1990s, the POMDP research community has been concerned primarily with finding efficient algorithms for solving POMDPs, which has led to different forms of approximate solution techniques. The previous section \autoref{approximations} surveyed the main approximations for POMDPs. These advances in theory have allowed POMDPs to start to be used in real world mission critical systems. This current section in the POMDP survey is focused explicitly on where POMDP theory may be applied with success. I seek to organize and present in a POMDP research hierarchy the versatility of the POMDP methodology.

\subsection{POMDP Basic Universal Model}
\begin{enumerate}
  \item Finite set of states $\mathpzc{X}=\{1,2,\ldots,n\}$.
  \item Finite set of controls $\mathpzc{U}=\{1,2,\ldots,U\}$.
  \item Finite set of observations $\mathpzc{Y}=\{1,2,\ldots,M\}$.
  \item A state to state transition function $p_{ij}(u) = Pr(X_{k+1}=j|X_k=i,U_k=u)$.
  \item A state to observation transition function $q_{jy}(u) = Pr(Y_{k+1}=y|X_{k+1}=j,U_k=u)$.
  \item A cost function, most generically defined on $\mathpzc{X} \times \mathpzc{U} \times \mathpzc{Y}$ as $c(i,u,y)$.
\end{enumerate}

In the above model $n, U, M$ are usually small positive integers. The state and observation transition probabilities are also usually put in matrices as before $P(u), Q_y(u)$. The immediate cost $c(i,u,y)$ is the most generic kind of cost function for this model because it considers not only the current state $x$ and control $u$ executed from $x$, but also any observation $y$ that can be observed. If observations are not relevant for the cost model, one can recast 6. as $c(i,u)$ so that the immediate cost is just a function of state and control.

Remember, the states are not directly observable to the agent or controller. The action set $U$ contains all of the choices or decisions that can be made at each stage. The observation set comprises all possible outputs the agent or controller can see at each stage. $p_{ij}(u)$ encodes the uncertainty in the state evolution while $q_{jy}(u)$ relates the outputs to the true system states. The cost function $c(i,u,y)$ gives the immediate cost signal for performing action $u$ in state $i$ and receiving observation $y$. The only goal is to use this model to learn a control policy $\mu(\pi)$ that yields the lowest total cost over all stages of decision making.

Now, I will present the modern POMDP research hierarchy. Cassandra originally had the categories of 1) Industrial Applications, 2) Scientific Applications, 3) Business Applications, 4) Military Applications, and 5) Social Applications. Some of these categories cast too wide of a net and are better broken into distinct categories that capture the essence of these application categories. Additionally, new categories must be added to accommodate the recent applications that have arisen in the last few decades. Below, the POMDP application hierarchy is enumerated.

\subsection{POMDP Application Hierarchy}

My categorization is as follows: 1) AI as a general discipline that encompasses POMDP theory and has many other applications for POMDPs, 2) Industrial Large-Scale applications: think factories or construction sites, 3) Robotics (autonomous cars, flying machines, humanoids, etc.), 4) Physical Sciences(Biology, Chemistry, Physics, 5) Business Applications, 6) Military Applications, 7) Financial(Monetary or Banking) and Economics Applications, 8) Social Applications, 9) Healthcare and Medicine, 10) Digital/Analog Communications(e.g. error-control coding), 11) Internet or Web perhaps, and perhaps 12) entertainment.
Need to do literature search to find other dominant recent trends here and see if anything exists for 4), 10), 11), and 12) and summarize the findings in the tables as the other categories. This will help the survey paper to shine, by adding so many of the recent trends in POMDP research, and make modeling assumptions accessible to a massive amount of researchers.

Now, I will start to present some sample tables to show how I will organize the material for these POMDP applications. First, I will create a listing consisting of the category name followed by a sub-listing of the problem instances. Then, I will provide a listing of the reference papers. Beneath the categorization, and reference papers, I will summarize the models for applications compactly in tabular form. Furthermore, I will include in table 1) a problem instance I have created for tracking a Moving Ship Target with communication issues that addresses the application areas of 10); Just, recently I came across the exciting POMDP application area of controlled sensing for POMDPs. This could be useful for my ship tracking problem based on how I am designing the problem.

%Category 1:

\subsection{POMDPs for AI}
\begin{enumerate}
   \item Artificial Intelligence (AI)
   \begin{enumerate}
     \item Machine Vision
     \item Dialog Management Systems
   \end{enumerate}
\end{enumerate}


1) Machine Vision and Visual Tracking:
Bandera, C.; Vico, F. J.; Bravo, J. M.; Harmon, M. E.; and III, L. C. B. 1996. Residual Q-Learning applied to visual attention. Machine Learning 20–27.

2) Visual Tracking:
Darrell, T., and Pentland, A. 1996. Active gesture recognition using partially observable Markov decision processes. In Thirteenth IEEE International Conference on Pattern Recognition (IPCR’96). Also appears as Technical Report No. 367 from M.I.T. Media Laboratory Perceptual Computing Section.

3) Dialogue Management Systems

One last example for POMDPs in AI: Spoken Dialogue Management Using Probabilistic Reasoning by Nicholas Roy and Joelle Pineau and Sebastian Thrun

The first two references may be useful for a ship tracking problem that I started to develop in the summer of 2020. New trends in control and communications point to an emerging field called Networked Controlled Systems. Rather than include my example of ship or "target" tracking in the AI table or the Military applications table, which it could be included in either table, I will present this example in the next section and start to discuss it further there. Chapter 6 will be where the discussion of NCS commences. In there, I will allude to places where POMDPs, in particular my examples and some new emergent theory could be applied from POMDPs to NCSs. In the next section, I will go over completely the ship tracking example, and start discussing any application papers that are relevant to the ship tracking example. After overviewing the ship tracking problem, in the final section of this chapter I will provide a review of the relevant papers to my own research similar to Chapter 2.

\newline
%\newpage
% \setlength{\arrayrulewidth}{1mm}
% \setlength{\tabcolsep}{10pt}
% \renewcommand{\arraystretch}{0.5}
%{\rowcolors{2}{green!80!yellow!50}{green!70!yellow!40}
\centering
\begin{tiny}
\begin{tabular}{ |p{2.5cm}|p{2.5cm}|p{2.5cm}|p{2.5cm}|p{3.0cm}|}
\hline
\multicolumn{5}{|c|}{Artificial Intelligence} \\
\hline
Problem Instance & States & Controls & Observations &  Costs\\
\hline
Machine Vision and Visual Tracking & states of the person or object to be tracked, e.g. handposition, facial expressions  & camera motions & feedback from particular areas the system is focused on & classification error of a gesture or expression class\\
\hline
Dialog Management Systems &  &  &  &  \\
\hline
\end{tabular}
\end{tiny}
%}

\subsection{POMDPs for Industrial Applications}
\begin{enumerate}
   \item Industrial Applications
   \begin{enumerate}
     \item Machine Maintenance
     \item Structural Inspection
     \item Elevator Control Policies
     \item Fishing Industry
   \end{enumerate}
 \end{enumerate}

% Second Table: Industrial Applicaitons
% Papers:
% 1) Read Monahan Survey of POMDPs for Machine Mainteance Discussion
% 2)

1) Machine Maintenance Papers:
Eckles, J. E. 1968. Optimum maintenance with incomplete information. Operations Research 16:1058–1067.
Ross, S. M. 1971. Quality control under Markovian deterioration. Management Science 17(9):587596.

2) Structural Inspection:
Ellis, H.; Jiang, M.; and Corotis, R. B. 1995. Inspection, maintenance, and repair with partial observability. Journal of Infrastructure Systems 1(2):92–99.

3) Elevator Control Policies:
Crites, R. H. 1996. Large-scale Dynamic Optimization Using Teams of Reinforcement Learning Agents. Ph.D. Dissertation, University of Massachusetts.

4) Fishery Industry:
Lane, D. E. 1989. A partially observable model of decision making by fishermen. Operations Research 37:240.

%\newpage
% \setlength{\arrayrulewidth}{1mm}
% \setlength{\tabcolsep}{10pt}
% \renewcommand{\arraystretch}{0.5}
%{\rowcolors{2}{green!80!yellow!50}{green!70!yellow!40}
\centering
\begin{tiny}
\begin{tabular}{ |p{2.5cm}|p{2.5cm}|p{2.5cm}|p{2.5cm}|p{3.0cm}|}
% \begin{supertabular}{ |p{2.75cm}|p{2.5cm}|p{2.5cm}|p{2.5cm}|p{3.0cm}|}
%\begin{tabularx}{ |X|X|X|X|X|}
\hline
\multicolumn{5}{|c|}{Industrial Applications} \\
\hline
Problem Instance & States & Controls & Observations &  Costs\\
\hline
Machine Maintenance & status of internal components  & observe output, inspect internals, repair, replace & product quality, inspection result & labor required, missed time, lost revenue\\
\hline
Structural Inspection(Roads and Bridges) & quality of material and parts & different inspections, replacements, adding reinforcements &  inspection results & higher costs for replacements, and less costs to add reinforcements or perform inspections \\
\hline
Elevator Control Policies & positions(possible floors), travel direction, number and location of passengers & where to send the elevator next, possibly skipping some people waiting & selections of call buttons inside the elevator and button presses at each floor, sensor measurements of occupants inside the elevator and waiting at the different floors & High costs for sensing hardware, total number of people waiting to be served, time waited. \\
\hline
Fishery Industry & actual population of different groups of fish & restocking, imposing fish bans, limits to fishing & results of local sample collections & near-term and long-term goals of the fishery, mainly success of managing population sizes. \\
\hline
\end{tabular}
\end{tiny}
%\end{tabularx}
%}

\subsection{POMDPs for Robotics}
\begin{enumerate}
   \item Robotics
   \begin{enumerate}
     \item Autonomous Vehicles
   \end{enumerate}
\end{enumerate}

Simmons, R., and Koenig, S. 1995. Probabilistic navigation in partially observable environments. In Fourteenth International Joint Conference on Artificial Intelligence, 1080–1087. Montreal, Canada: Morgan Kaufmann.


Cassandra, A.; Kaelbling, L.; and Kurien, J. 1996. Acting under uncertainty: Discrete bayesian models for mobile-robot navigation. In Proceedings of IEEE/RSJ International Conference on Intelligent Robots and Systems.


Cassandra, A. R.; Kaelbling, L. P.; and Littman, M. L. 1994. Acting optimally in partially observable stochastic domains. In Proceedings of the Twelfth National Conference on Artificial Intelligence, volume 2, 1023–1028. Menlo Park, California: American Association for Artificial Intelligence.


Nourbakhsh, I.; Powers, R.; and Birchfield, S. Summer 1995. Dervish: An office-navigating robot. AI Magazine 53–60.

%\newpage
% \setlength{\arrayrulewidth}{1mm}
% \setlength{\tabcolsep}{10pt}
% \renewcommand{\arraystretch}{0.5}
%{\rowcolors{2}{green!80!yellow!50}{green!70!yellow!40}
\centering
\begin{tiny}
\begin{tabular}{ |p{2.5cm}|p{2.5cm}|p{2.5cm}|p{2.5cm}|p{3.0cm}|}
\hline
\multicolumn{5}{|c|}{Robotics} \\
\hline
Problem Instance & States & Controls & Observations &  Costs\\
\hline
Autonomous Vehicles & robot location, configuration, surroundings, obstacles, internal state  & actuator usage & sensor readings, communications & success in meeting stated goals, e.g. cost is proportional to distance from goal\\
\hline
\end{tabular}
\end{tiny}


\subsection{POMDPs for The Physical Sciences}
\begin{enumerate}
   \item Physical Sciences (Biology/Chemistry/Physics and Astronomy):
   \begin{enumerate}
     \item Biology
     \item Chemistry
     \item Physics and Astronomy
   \end{enumerate}
\end{enumerate}

% Need to locate some papers for this hierarchy i thought of like chemical reactions, star or planet detection?

\subsection{POMDPs for Business Applications}
\begin{enumerate}
   \item Business Applications
   \begin{enumerate}
     \item Electrical Network Troubleshooting
     \item Distributed Database Queries
     \item Marketing Campaigns
     \item Questionaire Design
     \item Corporate Policy
   \end{enumerate}
\end{enumerate}

1) Electrical Network Troubleshooting: Thiebeaux, S.; Cordier, M.-O.; Jehl, O.; and Krivine, J.-P. 1996. Supply restoration in power distribution systems — a case study in integrating model-based diagnosis and repair planning. In Proceedings of the Twelfth Annual Conference on Uncertainty in Artificial Intelligence (UAI–96), 525–532.

2) Distributed Database Queries: Bayardo, R.; Bohrer, W.; Brice, R.; Cichocki, A.; Fowler, J.; Helal, A.; Kashyap, V.; Ksiezyk, T.; Mar- tin, G.; Nodine, M.; Rashid, M.; Rusinkiewicz, M.; Shea, R.; Unnikrishnan, C.; Unruh, A.; and Woelk, D. 1997. Infosleuth: An agent-based semantic integration of information in open and dynamic environ- ments. Proceedings of the ACM SIGMOD Interna- tional Conference on Management of Data.

3) Marketing Campaigns:
P. Rusmevichientong and B. Van Roy. A tractable POMDP for a class of sequencing problems. In Proc. of Uncertainty in Artificial Intelligence, 2001.

4) Questionaire Design
White, III, C. C. 1976. Optimal diagnostic question- aires which allow less than truthful responses. Infor- mation and Control 32:61–74.

5) Corporate Policy
Hughes, J. 1977. Optimal internal audit timing. Ac- counting Review LII:56–58.

Kaplan, R. 1969. Optimal investigation strategies with imperfect information. Journal of Accounting Re- search 7:32–43.

%\newpage
% \setlength{\arrayrulewidth}{1mm}
% \setlength{\tabcolsep}{10pt}
% \renewcommand{\arraystretch}{0.5}
%{\rowcolors{2}{green!80!yellow!50}{green!70!yellow!40}
\centering
\begin{tiny}
\begin{tabular}{ |p{2.5cm}|p{2.5cm}|p{2.5cm}|p{2.5cm}|p{3.0cm}|}
\hline
\multicolumn{5}{|c|}{Business Applications} \\
\hline
Problem Instance & States & Controls & Observations &  Costs\\
\hline
Electrical Network Troubleshooting & possible configurations of the network  & remotely operated electrical switches & noisy readings from limited number of circuit-breaker positions & customer satisfaction(No blackouts), time to locate faults\\
\hline
Distributed Database Queries & states of information sources(up, down, lightly loaded, heavily loaded, states of network components) & where to submit queries &  results of previous queries, general network traffic, specific network messages & costs with accessing certain info sources, preferences for response times of certain queries \\
\hline
Marketing(Internal Customer Model) & fits demographic or not, relevant attributes of person, likelihood of making a purchase, personality types & questions from a salesperson, or anything that elicits a customer reaction, different sales pitches (different offers) & customer reactions, consumer history, credit card purchases & missed sales, time spent with people that do not buy\\
\hline
Questionaire Design & type of person/customer & sequencing of the questions for the questionaire, or even picking different question sets & person's responses & amount of info extracted, proper info defined by questionaire's purpose.\\
\hline
Corporate Policy & true state of organization & performing audits, cost control & outcomes from audits & stability/productivity of organization.\\
\hline
\end{tabular}
\end{tiny}
%}


\subsection{POMDPs for Military Applications}
\begin{enumerate}
   \item Military Applications
   \begin{enumerate}
     \item Moving Target Search
     \item Target Identification
     \item Weapon Allocation
   \end{enumerate}
\end{enumerate}


1) Moving Target Search

Eagle, J. N. 1984. The optimal search for a moving target when the search path is constrained. Operations Research 32(5):1107–1115.

Pollock. 1970. A simple model of search for a moving target. Operations Research 18:883–903.

2)Target Identification

D’Ambrosio, B., and Fung, R. 1996. Far sighted approaches to sensor management experiments in reinforcement learning. Technical report, Prevision.

3) Weapon Allocation

Yost, K. A. 1998. Solution of sequential weapons allocation problems with imperfect, costly information. Presented at the Sixth INFORMS Computer Science Technical Section Conference.

%\newpage
% \setlength{\arrayrulewidth}{1mm}
% \setlength{\tabcolsep}{10pt}
% \renewcommand{\arraystretch}{0.5}
%{\rowcolors{2}{green!80!yellow!50}{green!70!yellow!40}
\centering
\begin{tiny}
\begin{tabular}{ |p{2.5cm}|p{2.5cm}|p{2.5cm}|p{2.5cm}|p{3.0cm}|}
\hline
\multicolumn{5}{|c|}{Military Applications} \\
\hline
Problem Instance & States & Controls & Observations &  Costs\\
\hline
Moving Target Search(e.g. Submarine Warfare, locating mobile missile platforms) & locations of the opposition's assets.  & selection of passive vs. active sonar, satellite camera re-positioning, reconnaissance flights, helicopter-based sonar sweeps & active measures available to try to detect the submarine e.g. using reconnaissance aircraft, satellite imagery, sonic buoys, surface vessels, etc. & how effective the search was (found vs. not fount), penalizing number and type of detection methods\\
\hline
Distributed Database Queries & states of information sources(up, down, lightly loaded, heavily loaded, states of network components) & where to submit queries &  results of previous queries, general network traffic, specific network messages & costs with accessing certain info sources, preferences for response times of certain queries \\
\hline
Target Identification(Hostile vs. Non-Threatening Aircraft Approachment) & attributes of the approaching aircraft: aircraft type, flying altitude, friendly vs. enemy, colors & selecting active vs. passive radar, launching or not launching intercept aircraft or surface-to-air missiles & results of sensing actions, perceived outcomes from actions & proportional to miss-classification rate, highly penalize friendly fire, reward adversarial death\\
\hline
Weapon Allocation(e.g. Aircraft with 2 air-to-surface missiles) & \# of missiles available at start of mission, \# of targets requested, damage level of targets & which target to strike first, whether a re-attack is necessary & recordings taken of the damage after the attack & based on priority of the targets, effectiveness of the attack(totally destroyed, some survivors, etc.)\\
\hline
\end{tabular}
\end{tiny}
%}

\newpage

\subsection{POMDPs for Finances and Economics}
\begin{enumerate}
   \item Finances and Economics
   \begin{enumerate}
     \item Inventory Control
     \item Dynamic Pricing Strategies
     \item Marketing Campaigns
   \end{enumerate}
\end{enumerate}

1) Inventory Control

J. T. Treharne and C. R. Sox. Adaptive inventory control for nonstationary demand and partial information. Management Science, 48(5):607–624, 2002.

2) Dynamic Pricing Strategies

Y. Aviv and A. Pazgal. A partially observed Markov decision process for dynamic pricing. Management Science, 51(9):1400–1416, 2005.

3) P. Rusmevichientong and B. Van Roy. A tractable POMDP for a class of sequencing problems. In Proc. of Uncertainty in Artificial Intelligence, 2001.

% \newpage
% \setlength{\arrayrulewidth}{1mm}
% \setlength{\tabcolsep}{10pt}
% \renewcommand{\arraystretch}{0.5}
%{\rowcolors{2}{green!80!yellow!50}{green!70!yellow!40}
\centering
\begin{tiny}
\begin{tabular}{ |p{2.5cm}|p{2.5cm}|p{2.5cm}|p{2.5cm}|p{3.0cm}|}
\hline
\multicolumn{5}{|c|}{Finances and Economics} \\
\hline
Problem Instance & States & Controls & Observations &  Costs\\
\hline
Inventory Control &   &  &  & \\
\hline
Dynamic Pricing Strategies &   &  &  & \\
\hline
Marketing Campaigns &   &  &  & \\
\hline
\end{tabular}
\end{tiny}
%}

\newpage

\subsection{POMDPs for Social Applications}
\begin{enumerate}
   \item Social Applications
   \begin{enumerate}
     \item Education
   \end{enumerate}
\end{enumerate}


1) Education

Karush, W., and Dear, R. 1967. Optimal strategy for item presentation in learning models. Management Science 13:773–785.

Smallwood, R. 1971. The analysis of economic teaching strategies for a simple learning model. Journal of Math Psych 8:285–301.

% \newpage
% \setlength{\arrayrulewidth}{1mm}
% \setlength{\tabcolsep}{10pt}
% \renewcommand{\arraystretch}{0.5}
%{\rowcolors{2}{green!80!yellow!50}{green!70!yellow!40}
\centering
\begin{tiny}
\begin{tabular}{ |p{2.5cm}|p{2.5cm}|p{2.5cm}|p{2.5cm}|p{3.0cm}|}
\hline
\multicolumn{5}{|c|}{Social Applications} \\
\hline
Problem Instance & States & Controls & Observations &  Costs\\
\hline
Education(teaching n concepts to an individual) & boolean indicating each concept learned or not  & various teaching strategies & test results given periodically & coverage of the required lesson plan, test scores, minimizing time to cover all the material, prioritization of certain material and thus weighting different test scores.\\
\hline
\end{tabular}
\end{tiny}
%}


\subsection{POMDPs for Healthcare and Medicine}
\begin{enumerate}
   \item Healthcare and Medicine
   \begin{enumerate}
     \item Robot Assisted Healthcare
     \item Medicine and Drug Therapies
     \item Healthcare Policy Making
   \end{enumerate}
\end{enumerate}

1) Robot Assisted Healthcare

J. Pineau, M. Montemerlo, M. Pollack, N. Roy, and S. Thrun. Towards robotic assistants in nursing homes: Challenges and results. Robotics and Autonomous Systems, 42(3–4):271–281, 2003b.


J. Boger, P. Poupart, J. Hoey, C. Boutilier, G. Fernie, and A. Mihailidis. A decision-theoretic approach to task assistance for persons with dementia. In Proc. Int. Joint Conf. on Artificial Intelligence, 2005.


M. Hauskrecht and H. Fraser. Planning treatment of ischemic heart disease with partially observable Markov decision processes. Artificial Intelligence in Medicine, 18:221–244, 2000.


C. Hu, W. S. Lovejoy, and S. L. Shafer. Comparison of some suboptimal control policies in medical drug therapy. Operations Research, 44(5):696–709, 1996.

2) HealthCare Policy Making

Smallwood, R.; Sondik, E.; and Offensend, F. 1971. Toward and integrated methodology for the analysis of health-care systems. Operations Research 19:1300– 1322.

% \newpage
% \setlength{\arrayrulewidth}{1mm}
% \setlength{\tabcolsep}{10pt}
% \renewcommand{\arraystretch}{0.5}
%{\rowcolors{2}{green!80!yellow!50}{green!70!yellow!40}
\centering
\begin{tiny}
\begin{tabular}{ |p{2.5cm}|p{2.5cm}|p{2.5cm}|p{2.5cm}|p{3.0cm}|}
\hline
\multicolumn{5}{|c|}{HealthCare and Medicine} \\
\hline
Problem Instance & States & Controls & Observations &  Costs\\
\hline
Robot-assisted healthcare & actual level of any given measured quantity, condition of patient  & conduct lab test, prescribe drugs, perform exploratory surgery, recommend different forms of physical therapy & What Physician sees after each action & treatment costs, patient health-risks, work time for the doctor.\\
\hline
 Health Care Policy Making & health status of varying populations of cities and states & how much money and where funds should be directed & sample health observations from the different regions & weigh short-term vs. long-term benefits, perhaps use average health measures as an indicator.\\
\hline
\end{tabular}
\end{tiny}
%}

==> Exact.tex <==
\section{Exact Methods for POMDPs}
\label{exact}
This will be by my estimation the longest chapter in terms of theory and overall number of papers that are reviewed in this survey. I will attempt to give coverage of all major approximation techniques for developing solutions to POMDPs since the 1980s to the present day. I will achieve this goal by breaking the approximation techniques down into their respective categories, and then reviewing the articles or dissertations that comprise that given technique category, mostly chronologically. Also, any techniques that will be useful for the Markovian moving target tracking application or the Markovian source for error correction problems will also be considered. These techniques will be considered for usage in for the above applications but in the context of Networked-Control Systems in another chapter, i.e. for distributed multi-agent control.

I will start with the class of exact algorithms for POMDPs and then, swiftly focus attention on the approximation methods that have been developed. The reasons for approximation techniques for POMDPs are clear at this point in the survey of POMDP techniques. Intractability and computational burden are with us in the general case. As such, the next section will focus attention on reduction to MDP from POMDP techniques. Then, I will discuss the second category of approximation methods that will be reviewed for my literature review paper, i.e, grid-based techniques.

Later, after I finish my paper count requirements for my literature review paper, I will circle back and review more papers around a few other approximation methods. Firstly, I will review the class of gradient descent methods that are already used in the field of RL in different algorithms. Within this area, I am academically interested in the theory of function approximation approaches for solving POMDPs as this is heavily used in RL, and I am already familiar with the families of theories from RL that encompass function approximation. These have the potential to solve challenging continuous state and continuous control problems under large amounts of uncertainty. The last few techniques I will review are compression methods for POMDPs, Search in Policy Space, and speculate as well as comb the literature on a number of other heuristic based optimization approaches that could be useful for developing baselines in heuristics for more challenging POMDP domains. As I review the research articles I will point out places for extensions, and discuss places where the research is sparse, and ultimately look for ways to apply these methods to my applications.

A solution in terms of a policy to a POMDP is in general a mapping from belief space to action space. In the notation I have used throughout the survey, that analytically means $u=\mu(\pi)$. An optimal policy is characterized by a cost-to-go function for minimization of costs as $J_\mu(\pi_0)= E[\sum_{k=0}^{\infty} \gamma^k c(\pi_k,\mu(\pi_k))]$ for some stationary policy $\mu$. In general, one could insert $\mu_k$ in place of $\mu$ for a non-stationary policy. Even for a finite horizon, the POMDP has proven to be P-SPACE complete. For this reason, most applications rely on a simplified MDP-based approximation. These reasons again show how complex it is to develop an exact solution to a POMDP. This calls us to develop the best approximation techniques that are possible. First I will cover some techniques from papers that deal with exact methodology, and then I will review papers from the already mention two categories of approximations: reduction to MDP from POMDP and grid-based methods. Within the category of exact methods, I will cover those papers that use exact methods that focus on value iteration for POMDPs and then exact methods that rely on pruning the set of alpha vectors to decrease computational burdens.

\subsection{Exact Methods with Pruning Strategies}

All exact methods stem from the classical papers we have already studied in Chapter 3, particularly the work of Sondik. Remember, at each stage $k$ we were able to iteratively construct a set of alpha vectors $A_k$ from the future stage. See Krish17 p.158 for more on a general incremental pruning algorithm. On the next page of that text, he also explains how the prune function works. It comes from testing whether or not an alpha vector dominates every other vector in the set of alpha vectors minus the vector being tested of course. Effectively, we need to check if $\exists\ \alpha \in A_k$ such that $\forall b \in B(X)\  \alpha^T b \geq \bar{\alpha} b\  \forall \bar{\alpha} \in A_k - \{\alpha\}$. If this holds, then $\alpha$ dominates every other alpha vector in  $A_k$ and will never contribute to the Cost-to-go function, i.e., it is never active.

The paper by Monahan, "A survey of partially observable Markov decision proceses: Theory, models and algorithms" Management Science, 28(1), January 1982, computes the set of $\alpha$ vectors $A_k(u)$ at each stage which has $|U||A_{k+1}|^Y$ alpha vectors in it, where $Y$ is the number of possible observations and the other are cardinalities of finite sets. These are pruned according to the linear program which Krish17 presents on p.159 of his textbook. Monahan also goes over an enumeration strategy for value iteration for POMDPs, but in general, as we have already seen, the problem grows exponentially in the number of alpha vectors used to approximate the value function. This necessitates the use of pruning strategies for large state problems to save on vast quantities of useless computations.

The witness algorithm is main one that computes the exact value funciton with the exact belief state, but it is really ugly looking. It is motivated in the following paper, and references to other approximation papers are given and will be detailed in the next section of this survey paper.

Paper # 6 "Acting Optimally in Partially Observable Stochastic Domains."-by Anthony R. Cassandra et. al.

\subsection{Acting Optimally in Partially Observable Stochastic Domains}

This paper is all about presenting a new more computationally efficient algorithm for finding POMDP's optimal policies, called the Witness algorithm. However, the details of this algorithm are left to a separate technical report. Some results are given from this algorithm and a few simple toy models are given.

First, I would like to recast her approach into cost minimization from reward maximization and continue with our notation already developed. No new notation is required for reading and understanding this paper. In this paper, an interesting block-diagram illustrates the dynamics of a POMDP. The dynamics show $y$ an observation, $b$ a belief-state, and $u$ a control being input into the "S.E." block, which stands for state estimator. "S.E." produces a new belief state. This is the optimal Bayesian filter we have studied several times already.

For POMDPs, since the states are not completely observable, we can only learn about them through the observation process. Given a finite set of observations $\mathzpc{Y} = \{1,2,...,M\}$, we have a discrete PMF over $\mathzpc{Y}$ given by $Pr(Y=y|X=x, U=u)$ which is the probability of observing $y$ given the true current state is $x$ and we choose $u$ in the previous period. Another common notation for belief-state is $b$. $b$ models the internal belief of the true state $x$ as the component $b(x)$. The other component in the figure is the policy which maps $b \to \mathzpc{U}=\{1,2,..,U\}$, where $U$ is the finite set of actions which is the same as in our basic universal model of POMDPs.

The formula for $b'(x')$, i.e., the belief of state $x'$ at the next stage is:
$$ b'(x') = \frac{q_{x'y}(u)\sum_{x}P_u(x,x')b(x)}{\sum_{x'}q_{x'y}(u)\sum_{x}P_u(x,x')b(x)} ,$$ is our formula for SE given our transition models, observation transition probabilities, and the previous belief-state.

Next, is presented in the paper a simple POMDP environment that has 4 states layed out on a line as 4 adjacent boxes, 1 of which is a goal state. The other 3 are not goal states, and no cost is incurred in them. At the goal state say a cost of -1 is achieved. From any state, the agent can move left e.g. $u=0$, or right, say $u=1$. If the agent runs into a wall the agent stays in the same state. Once the agent reaches $x=2$, the goal state, the agent with equal probability is placed in either $0, 1,$ or $3$. A small back of the envelope calculation for updating the belief state is then given to see how $b_k$ changes over time.

An example of a type of reduction approach is based on using the belief state with a Q function based on the Q-learning algorithm of Watkins and Dayan is denoted as $Q^*_{CO}$. CO stands for completely observable. Here, this would be the optimal state-action cost for us based on the completely observable MDP $(\mathzpc{X},\mathzpc{U},P_u(x,x'),c(x,u),\gamma)$. Given a belief-state $b$, generate the control $u$ s.t.  $$\arg\min\limits{u\in \mathzpc{U}} \sum_{x}b(x)Q^*_{CO}(x,u). $$ This pretends that the stochasticity is only present for the immediate stage and that the environment is CO for all future stages. The main issue with this type of reduction is that this kind of approximation can lead to policies that do not explore much or seek to gain more information.

Paper refereneces:
Paper # 6 "Technical Note Q-Learning", by Christopher Watkins, et. al.

Paper # 6 will be reviewed in the reduction section and the following paper will be surveyed about perceptual aliasing:

Paper # 7 "Reinforcement learning with perceptual aliasing: the perceptual distinctions approach", by Lonnie Chrisman
Each of these papers will be reviewd after the current paper is reviewed as they have real value for research.

The already proven way to find optimal policies is to recast the POMDP as a continuous state MDP with $b$ as the state. For any action $u$ and belief $b$, there are only $|Y|=M$ successor beliefs $b'$ that are possible. With this in mind, define a new belief-state transition function as $$ \tau(b,a,b') = \sum\limits_{y\in\mathzpc{Y}:SE(b,u,y)=b'}Pr(y|u,b).$$ Define the cost function as $$ \rho(b,u) = \sum\limits_{x\in\mathzpc{X}}b(x)c(x,u) .$$ This allows the agent to minimize costs using its current belief-state. The agent cannot fool itself by the design of S.E.

Next, the method of Value Iteration for discounted infinite horizon for POMDPs is presented. The optimal cost-to-go from any belief $b$ is the infinite expected sum of discounted costs starting in state $b$ and executing the optimal policy. The optimal cost-to-go $J^*(b)$ can be expressed as a system of simulatenous equations analgously to the Bellman equations of MDPs:
$$ J^*(b) = \min\limits_{u\in U}[\rho(b,u) + \gamma \sum_{b'\in B}\tau(b,u,b')J^*(b')] .$$

One could consider value iteration for a finite horizon, but it is known that in the limit that $J^*_k(b) \to J^*(b)$ approaches the infinite-horizon cost-to-go function, where $k$ is the number of stages. Then, VIA is presented as:
\begin{algorithm}[H]
\SetAlgoLined
\KwResult{Converged cost-to-go function within $\epsilon$ optimality}
 Let\  $J_0(b)=0\  \forall b\in B$\;\newline
 Let\  $k=1$\;\newline
 \For{$b\in B$}{
      $J_1(b) = \max\limits_{u\in U}[\rho(b,u) + \gamma \sum\limits_{b'\in B}\tau(b,u,b')J_{0}(b')$\;
    }
 $J_1(b) = \max\limits_{u\in U}[\rho(b,u) + \gamma \sum\limits_{b'\in B}\tau(b,u,b')J_0(b')]$\;\newline
 \While{$|J_k(b)-J_{k-1}(b)| < \epsilon$}{
        Let\  $k += 1$\;\newline
      \For{$b\in B$}{
      $J_k(b) = \max\limits_{u\in U}[\rho(b,u) + \gamma \sum\limits_{b'\in B}\tau(b,u,b')J_{k-1}(b')]$\;
    }

 }
 \caption{VIA for POMDPs}
\end{algorithm}

She references Lovejoy for more on this technique.
Paper # 8 Lovejoy 1991. It converges in a finite number of steps and policy yields a value function that is within $\frac{2\gamma\epsilong}{(1-\gamma)}$ of the optimal policy.

Paper # 8
Lovejoy, W. S. 1991. A survey of algorithmic methods for partially observed markov decision processes. Annals of Operations Research 28(1):47-65.

Next, they discuss briefly, the Witness Algorithm, and explain linear representations of $J_k(\cdot)$ that comes from Sondik's work. The essence of it is to design a linear program that returns a single point that is a "witness" to the fact that $\hat{J}_t \neq J^*_t$. This is in a separate report, and I may take notes on it, but I have also read in Krish Ch.7 that Lovejoy's exact method can perform better than Witness by a constant factor so I will instead review that paper in the Exact Methods Section.

There is one other interesting idea in the current paper by Cassandra. Representation of policies as policy graphs is presented next and a new toy model problem is given called the Tiger Problem. See the toy models chapter 4 for more on this toy model problem and a host of other toy model problems. On representing policies: If we let $\nu_t$ be a set of $|\mathzpc{X}|$-dimensional vectors of real numbers, the optimal $k$-stage cost-to-go functions can be written as $$J_t(b) = \max\limits_{\alpha\in \nu_t} b\cdot \nu_t .$$ The policy graph succintly describes the final optimal policy based on the final partitioning of the belief-space. For more on policy graph, refer directly to the paper, "Once computed, the policy graph is a representation of the optimal policy. The agent chooses the action associated with the start node, and then, depending on which observation it makes, the agent makes a transition to the appropriate node. It executes the associated action, follows the arc for the next observation, and so on."

\subsection{Lovejoy, W. S. 1991. A survey of algorithmic methods for partially observed markov decision processes.}




Another paper came along by A. R. Cassandra which according to Krish17 developed an algorithm that is better than the Witness algoirthm by a constant factor so I will review that paper also.

Paper # 9
The paper is titled, "Incremental pruning: A simple fast exact method for partially observed Markov decision processes." In proceedings of the 13th Annual Conference on Uncertainty in Artificial Intelligence (UAI-97).
\subsection{Incremental pruning: A simple fast exact method for partially observed Markov decision processes.}





Another interesting result that comes from running value iteration on POMDPs, in terms of accuracy of the value function is the following: $$ |V_N(\pi)-V(\pi)| \leq \frac{\rho^{N+1}}{1-\rho}\max\limits_{x,u}|c(x,u)|, $$ where the error is based on having run value iteration for $N$ stages, a discount factor $\rho$ and the maximum value of the cost table. See section $7.6.3$ of Krish17 for more details.

The rest of the focus in this chapter is on reduction to MDP techniques from the POMDP and separately, grid-based techniques. The objective will be review other highly accurate, computationally friendly algorithms that can achieve near-optimal policies while still giving us plenty of insight into the POMDP problem we are trying to solve. Other categories papers will be only listed for the time being. Within the first two major categories there has been enough successful research that needs to be reviewed and understood so I can apply the best techniques later to my applications, both target tracking and error correction of Markovian sources and channels, as well as to the emerging field of Networked Control Systems (NCSs) which is where the future directions of the control community is pointing. For NCS, specifically I am referring to control in a distributed sense, not control of the network, which is a separate research area, but rather I am referring to control of sensors, controllers, and actuators through usage of a network. Chapter 6 will go into detail On NCS and the issues there. I will review a number of papers that I have found for this field that have helped to establish in within the control community.

==> Introduction.tex <==
\section{Introduction}

